A Flux-Differencing Formula for Split-Form Summation By Parts Discretizations of Non-Conservative Systems: Applications to Subcell Limiting for magneto-hydrodynamics

In this paper, we show that diagonal-norm summation by parts (SBP) discretizations of general non-conservative systems of hyperbolic balance laws can be rewritten as a finite-volume-type formula, also known as flux-differencing formula, if the non-conservative terms can be written as the product of a local and a symmetric contribution. Furthermore, we show that the existence of a flux-differencing formula enables the use of recent subcell limiting strategies to improve the robustness of the high-order discretizations. To demonstrate the utility of the novel flux-differencing formula, we construct hybrid schemes that combine high-order SBP methods (the discontinuous Galerkin spectral element method and a high-order SBP finite difference method) with a compatible low-order finite volume (FV) scheme at the subcell level. We apply the hybrid schemes to solve challenging magnetohydrodynamics (MHD) problems featuring strong shocks.

==> hybridized_SBP.tex <==
\section{Hybridized SBP formulation}

In this section, we describe the formulation of the entropy stable Gauss collocation scheme in one dimension using ``hybridized'' summation-by-parts operators \cite{chen2020review}. Formulations using hybridized operators are similar to formulations using traditional SBP operators, but are equivalent to the formulation (\ref{eq:Gauss_DGSEM_cons}) which introduce additional surface terms. 

First, we define the matrix $\mat{V}_h$ 
\[
\mat{V}_h = \begin{bmatrix}
\mat{I}\\
\mat{V}_f
\end{bmatrix} \in \mathbb{R}^{N+3, N+1}
\]
Multiplication by $\mat{V}_h$ maps nodal values at Gauss nodes to the vector containing nodal values at \textit{both} Gauss nodes and face nodes. Next, we introduce the hybridized SBP operator
\[
\mat{Q}_h = \frac{1}{2}\begin{bmatrix}
\mat{S} & \mat{V}_f^T\mat{B}\\
-\mat{B}\,\mat{V}_f & \mat{B}
\end{bmatrix}
\]
where we have used the skew-symmetric matrix $\mat{\hat{S}} = 2\mat{Q}-\mat{V}_f^T\mat{B}\,\mat{V}_f = \mat{Q}-\mat{Q}^T$. The operator $\mat{Q}_h$ satisfies a generalized SBP property and can be used to construct degree $N$ approximations to derivatives \cite{chan2019efficient}. 

We now introduce the skew-symmetric hybridized matrix $\mat{\hat{S}}_h = \mat{Q}_h - \mat{Q}_h^T$. Then, (\ref{eq:Gauss_DGSEM_GLMMHD}) can equivalently be formulated as
\begin{empheq}[box=\fbox]{align}
J \omega_j \dot{\state{u}}_j 
+ \sum_{k=0}^{N+2} 2 {V}_{h, kj} & \state{r}_{h,k}
+ \sum_{k=0}^N \left({V}_f\right)_{kj} \state{s}_k
= \state{0},  \label{eq:Gauss_hybridized_noncons}
\end{empheq}
where $\state{r}_{h,k}, \state{s}_k$ are volume and surface contributions computed in terms of the hybridized SBP operator 
\begin{empheq}[box=\fbox]{align}
\state{r}_{h,j} = \sum_{k=0}^{N+2} {\hat{S}}_{h, jk} \left(\state{f}^{*}_{(j,k)} + \numnonconsD{\Jan}_{(j,k)} \right), \qquad
\state{s}_j = \delta_{jN}
\left( \numfluxb{f}^a_{(N,R)} + \numnonconsD{\Jan}_{(N,R)} \right)
-\delta_{j0}\left( \numfluxb{f}^a_{(0,L)} + \numnonconsD{\Jan}_{(0,L)}  \right).
\end{empheq}
Note that, in contrast to (\ref{eq:Gauss_DGSEM_GLMMHD}), the formulation (\ref{eq:Gauss_hybridized_noncons}) combines the additional local surface terms into the definition of the volume operator. The resulting contributions $\state{r}_h$ and $\state{s}$ more closely resemble the simpler LGL formulation (\ref{eq:LGL_DGSEM_GLMMHD_cleanedUp}).

To show equivalence, we first note that since the entries of $(\mat{V}_f)_{1j}$ and $(\mat{V}_f)_{2j}$ are $\ell_j(-1)$ and $\ell_j(+1)$, the surface term $\sum_{k=0}^N \left({V}_f\right)_{kj} \state{s}_k$ can be rewritten as
\begin{equation}
-\ell_j(-1) \left( \numfluxb{f}^a_{(0,L)} + \numnonconsD{\Jan}_{(0,L)}  \right)
+ \ell_j(+1)\left( \numfluxb{f}^a_{(N,R)} + \numnonconsD{\Jan}_{(N,R)} \right).
\label{eq:hybridized_1}
\end{equation}
Next, we split the since the contribution $\sum_{k=0}^{N+2} 2 {V}_{h, kj} \state{r}_{h,k}$ into two parts. Note this can be written equivalently as a matrix-vector product
\begin{equation*}
\mat{V}_h^T \state{r}_h = \begin{bmatrix}
\mat{I} \\
\mat{V}_f
\end{bmatrix}^T \begin{bmatrix}
\state{r}\\
\state{r}_f
\end{bmatrix} = \state{r} + \mat{V}_f^T\state{r}_f.
\end{equation*}
upper left block of $\mat{\hat{S}}_h$ is the skew symmetric part of the generalized SBP operator $\mat{\hat{S}}$, one can write the entries of the contribution $\state{r}_j$ as
\begin{equation}
\sum_{k=0}^N \hat{S}_{jk} \left(\state{f}^{*}_{(j,k)} + \numnonconsD{\Jan}_{(j,k)} \right) - \ell_j(-1)\left(\state{f}^{*}_{(j,k)} + \numnonconsD{\Jan}_{(j,k)}\right) + \ell_j(+1)\left(\state{f}^{*}_{(j,k)} + \numnonconsD{\Jan}_{(j,k)}\right).
\label{eq:hybridized_2}
\end{equation}
Finally, we consider the contribution $\mat{V}_f^T\state{r}_f$. The term $\state{r}_f$ is equivalent to 
\begin{align*}
\state{r}_{f,j} &= \sum_{k=0}^N -\delta_{j0}\ell_k(-1)\left(\state{f}^{*}_{(L,k)} + \numnonconsD{\Jan}_{(L,k)}\right) + \delta_{jN}\ell_k(+1)\left(\state{f}^{*}_{(R,k)} + \numnonconsD{\Jan}_{(R,k)}\right) \\
&=\sum_{k=0}^N -\delta_{j0}\ell_k(-1)\left(\state{f}^{*}(\tilde{\state{u}}_L,\state{u}_k) + \numnonconsD{\Jan}(\tilde{\state{u}}_L,\state{u}_k)\right) + \delta_{jN}\ell_k(+1)\left(\state{f}^{*}(\tilde{\state{u}}_R,\state{u}_k) + \numnonconsD{\Jan}(\tilde{\state{u}}_R,\state{u}_k)\right) 
\end{align*}
Multiplication by $\mat{V}_f^T$ then yields 
\begin{equation}
\mat{V}_f^T\state{r}_{f} = -\ell_j(-1)\left(\sum_{k=0}^N \ell_k(-1)\left(\state{f}^{*}(\tilde{\state{u}}_L,\state{u}_k) +
\numnonconsD{\Jan}(\tilde{\state{u}}_L,\state{u}_k)\right)\right) + 
\ell_j(+1) \left(\sum_{k=0}^N\ell_k(+1)\left(\state{f}^{*}(\tilde{\state{u}}_R,\state{u}_k) + \numnonconsD{\Jan}(\tilde{\state{u}}_R, \state{u}_k)\right)\right).
\label{eq:hybridized_3}
\end{equation}
Combining (\ref{eq:hybridized_1}), (\ref{eq:hybridized_2}), and (\ref{eq:hybridized_3}) then recovers the Gauss-DGSEM formulation for GLM-MHD (\ref{eq:Gauss_DGSEM_GLMMHD}). 
% Multiplying by $\mat{V}_f^T$ then yields
% \begin{align*}
% \mat{V}_f^T\state{r}_f &= 

% \sum_{k=0}^N -\ell_k(-1)\left(\state{f}^{*}(\tilde{\state{u}}_L,\state{u}_k) + \numnonconsD{\Jan}(\tilde{\state{u}}_L,\state{u}_k)\right) + \ell_k(+1)\left(\state{f}^{*}(\tilde{\state{u}}_R,\state{u}_k) + \numnonconsD{\Jan}(\tilde{\state{u}}_R,\state{u}_k)\right) 
% \end{align*}
% \change{TODO: add equivalence.}


% Noting that we can simplify for LGL nodes, Bohm's version can be rewritten as:
% \begin{empheq}[box=\fbox]{align} 
% J \omega_j \dot{\state{u}}_j 
% + \state{r}_j
% + \sum_{k=0}^N \mat{V}_{f,kj} \state{s}_k
% = \state{0}.
% \end{empheq}
% Here, the surface contribution $\state{s}$ is identical to the Gauss case, and the volume contribution is
% \[
% \state{r}_j = \sum_{k=0}^N S_{jk} \left( \state{f}^{*}_{(j,k)} + \numnonconsD{\Jan}_{(j,k)} \right)
% \]
